The Smart Sampling Kalman Filter with Symmetric Samples

Nonlinear Kalman Filters are powerful and widely-used techniques when trying to estimate the hidden state of a stochastic nonlinear dynamic system. In this paper, we extend the Smart Sampling Kalman Filter (S2KF) with a new point symmetric Gaussian sampling scheme. This not only improves the S2KF's estimation quality, but also reduces the time needed to compute the required optimal Gaussian samples drastically. Moreover, we improve the numerical stability of the sample computation, which allows us to accurately approximate a thousand-dimensional Gaussian distribution using tens of thousands of optimally placed samples. We evaluate the new symmetric S2KF by computing higher-order moments of standard normal distributions and investigate the estimation quality of the S2KF when dealing with symmetric measurement equations. Finally, extended object tracking based on many measurements per time step is considered. This high-dimensional estimation problem shows the advantage of the S2KF being able to use an arbitrary number of samples independent of the state dimension, in contrast to other state-of-the-art sample-based Kalman Filters.

==> Sections/Acknowledgment.tex <==

\section{Acknowledgment}


